Approximate Multi-Matroid Intersection via Iterative Refinement

We introduce a new iterative rounding technique to round a point in a matroid polytope subject to further matroid constraints. This technique returns an independent set in one matroid with limited violations of the other ones. On top of the classical steps of iterative relaxation approaches, we iteratively refine/split involved matroid constraints to obtain a more restrictive constraint system, that is amenable to iterative relaxation techniques. Hence, throughout the iterations, we both tighten constraints and later relax them by dropping constrains under certain conditions. Due to the refinement step, we can deal with considerably more general constraint classes than existing iterative relaxation/rounding methods, which typically round on one matroid polytope with additional simple cardinality constraints that do not overlap too much. We show how our rounding method, combined with an application of a matroid intersection algorithm, yields the first $2$-approximation for finding a maximum-weight common independent set in $3$ matroids. Moreover, our $2$-approximation is LP-based, and settles the integrality gap for the natural relaxation of the problem. Prior to our work, no better upper bound than $3$ was known for the integrality gap, which followed from the greedy algorithm. We also discuss various other applications of our techniques, including an extension that allows us to handle a mixture of matroid and knapsack constraints.

==> apps-condensed.tex <==
\section{Further applications and extensions} \label{apps}

\vspace*{-1ex}
%\paragraph{{\bf Spanning tree with matroid constraints.}} 
%Consider the following 
\paragraph{{\bf Generalized matroidal degree-bounded spanning tree \sc (gmdst)}.}
In this problem, we are given an undirected graph 
$G=(V,E)$ with edge costs $c\in\R^E$, disjoint node-sets $S_1,\ldots,S_k$, and
matroids $M_i=(\dt(S_i),\I_i)\;\forall i=[k]$, where $\dt(S_i)$ is the edge set of
$G$ crossing $S_i$. We want to find a spanning tree $T$ of minimum cost such that
$T\cap\dt(S_i)\in\I_i\;\forall i\in [k]$. This generalizes matroidal
degree-bounded MSTs considered by~\cite{zenklusen_2012_matroidal}, 
%(which itself generalizes degree-bounded MST),
wherein each node $\{v\}$ is an $S_i$ set.
Clearly, each edge belongs to at most $2$ ground sets of the matroids $\{M_i\}_{i \in [k]}$.
Thus, by taking $M_0$ to be the graphic matroid 
and setting $w=-c$, Theorem~\ref{thm:mainthm} leads to a tree $T$ of cost at most the optimum such that 
$T\cap\dt(S_i)$ is $2$-independent in $M_i \;\forall i\in [k]$. 

\begin{comment}
Complementing this, we show in Appendix~\ref{addviol}, via the same replication idea used
to rule out an additive violations for \eqref{eq:baseQMatchoid}, that an additive
violation of the matroid constraints is impossible in polytime for \gmdst. 
This is in stark contrast with the result of~\cite{zenklusen_2012_matroidal},
who obtains an $O(1)$ additive violation for the special case of
of matroidal degree-bounded MST problem.
\end{comment}

We remark that, whereas~\cite{zenklusen_2012_matroidal} obtains an $O(1)$ {\em additive}
violation of the matroid constraints for matroidal degree-bounded MST
problem, %we show in Appendix~\ref{addviol} that 
such a polytime additive guarantee is not possible for \gmdst. 
This follows from the same replication idea used to rule out additive
violations for \eqref{eq:baseQMatchoid}. %in Appendix~\ref{addviol}. 

\vspace*{-1ex}
\paragraph{{\bf Extension to knapsack constraints.}}
We can consider a generalization of \eqref{eq:baseQMatchoid}, where, in addition to
the matroids %constraints involving matroids 
$M_0, \dots, M_k$ (over subsets of $N$) and weight vector $w\in\R^N$, we have $t$ knapsack 
constraints, indexed by $i = k + 1, \dots, k + t$. The $i$-th knapsack constraint is
specified by a ground set $N_i\sse N$, cost vector $c^i\in\mathbb{R}^{N_i}_{\geq 0}$, and budget
$U_i\geq 0$.  
The goal is to find a maximum-weight set $R$ such that
$R\in\base_0\cap\I_1\cap\ldots\cap\I_k$, and satisfying $c^i(R\cap N_i)\leq U^i$ for all
$i=k+1,\ldots,k+t$. 

\begin{comment}
We may assume %without loss of generality that $C^i := \max_{e \in N_i}
that $c^i_e \le U_i$ for all $e$ (as otherwise, $e$ cannot belong to any feasible
solution, and can be deleted).
\end{comment}

\begin{comment}
(If this inequality did not hold, then we could identify and drop some
elements that do not belong to any feasible solution.) 
We consider the following problem 
\begin{equation}\label{eq:baseQMatchoid_knapsack}
%\max\ \bigl\{w(I): \ I\in \mathcal{I}_i \ \ \forall i=0,\ldots,k, \quad |I\cap N_0|\geq L, c^i(I \cap N_i) \le U_i \ \ \forall i = k + 1, \ldots, k + t\bigr\}\;.
\max\ \bigl\{w(I): \ I\in \base_0, \;\; I \in \I_i \ \  \forall i \in [k], \;\; c^i(I \cap
N_i) \le U_i \ \ \forall i = k + 1, \ldots, k + t\bigr\}\;. 
\end{equation}
\end{comment}

We consider the natural LP-relaxation \eqref{eq:knapLP} for this problem, and extend
Theorem~\ref{thm:mainthm} to obtain the following result; we sketch the proof in
Appendix~\ref{append-proofs}. 

\begin{theorem} \label{thm:knapThm} \label{thm:knapthm}
\begin{comment}
Consider the following LP-relaxation of the above problem.
\begin{align*}\label{eq:knapLP}
\max\ \Bigl\{w^Tx: \ \ & x\in\R^N, \quad x\vert_{N_0}\in P_{\base_0}, \quad
x\vert_{N_i}\in P_{\I_i}\ \ \forall i\in[k], \\
& (c^i)^Tx\vert_{N_i} \le U_i\ \ \forall i=k+1, \ldots, k+t\quad \Bigr\}.
\tag{\LPKnapsack}
\end{align*}
\end{comment}
Let $q_1,\ldots, q_{k + t} \in \mathbb{Z}_{\geq 1}$ be such that 
%\begin{equation}\label{eq:loadPropKnap}
$\sum_{i\in [k + t]: e\in N_i} \frac{1}{q_i} \leq 1$ for all $e\in N$.
%\espace.
%\end{equation}
%\noindent
If \eqref{eq:knapLP} is feasible, then one can efficiently compute $R \subseteq N$ such that
\begin{enumerate*}
\item $R\in\base_0$; \label{prop_knap_first}
%\item $|R\cap N_0|\geq L$;
\item $w(R)\geq\OPT_{\text{\ref{eq:knapLP}}}$; %is no more than the optimal value of~\eqref{eq:mainLP}; 
%\item $R \in \mathcal{B}_0$; and
\item $R$ is $q_i$-independent in $M_i$ for all $i \in [k]$; and \label{prop_knap_second_to_last} %$\chi^R\in q_iP_{\I_i}$, or equivalently, $R\cap N_i$ can be partitioned into $q_i${}
  %independent sets of $M_i$, for all $i\in[k]$; and \label{prop_knap_second_to_last}
\item $c^i(R \cap N_i) \le U_i + q_i\cdot\bigl(\max_{e\in N_i}c^i_e\bigr)$
%$\le (q_i + 1) U_i$ 
for all $i\in\{k + 1, \dots, k + t\}$. \label{prop_knap_last}
\end{enumerate*}
%
%\noindent 
%In particular, taking $q_i=\Dt\coloneqq\max_{e\in N}\bigl|\{i\in[k + t]: e\in N_i\}\bigr|$ for
%all $i\in[k + t]$, we have that $R \cap N_0$ is an independent set of $M_0$ of the required size;
%$R \cap N_i$ is $\Dt$-independent in $M_i$ for all $i\in[k]$; and $R$ violates knapsack constraint $i$ by at most a factor of $\Delta + 1$, for all $i \in \{k+1, \dots, k+t\}$. 
\end{theorem}


